Scaling Quantum Computations via Gate Virtualization

We present the Quantum Virtual Machine (QVM), an end-to-end generic system for scalable execution of large quantum circuits with high fidelity on noisy and small quantum processors (QPUs) by leveraging gate virtualization. QVM exposes a virtual circuit intermediate representation (IR) that extends the notion of quantum circuits to incorporate gate virtualization. Based on the virtual circuit as our IR, we propose the QVM compiler - an extensible compiler infrastructure to transpile a virtual circuit through a series of modular optimization passes to produce a set of optimized circuit fragments. Lastly, these transpiled circuit fragments are executed on QPUs using our QVM runtime - a scalable and distributed infrastructure to virtualize and execute circuit fragments on a set of distributed QPUs. We evaluate QVM on IBM's 7- and 27-qubit QPUs. Our evaluation shows that using our system, we can scale the circuit sizes executable on QPUs up to double the size of the QPU while improving fidelity by 4.7$\times$ on average compared to larger QPUs and that we can effectively reduce circuit depths to only 40\% of the original circuit depths.

==> tables/benchmarks.tex <==
\begin{table}[t]
\centering
\begin{tabular}{ |p{5.3cm}|p{1.4cm}| }
\hline
{\bf Description} & {\bf Name} \\
\hline
\hline
GHZ \cite{tomesh2022supermarq} & ghz  \\
\hline
Hamiltonian Simulation \cite{tomesh2022supermarq} & hamsim-$l$ \\
\hline
Variational Quantum Eigensolver (VQE) \cite{tomesh2022supermarq} & vqe-$l$ \\
\hline
TwoLocal ansatz (Ising) \cite{quetschlich2022mqt} & 2local-$l$ \\
\hline
Quantum Approximate Optimization (QAOA) \cite{quetschlich2022mqt} & qaoa-$d$ \\
\hline
Approx. Quantum Fourier Transform \cite{quetschlich2022mqt} & aqft-$d$ \\
\hline

% \hline
% vqe($r$) &  \\
% \hline
% ham\_sim($r$) & \\
% \hline
% 2local($r$) & \\
% \hline
% qaoa($d$) & For our evaluation we use regular $d$-graphs with $d \in \{3, 4\}$ \\
% \hline
% aqft($a$) &  \\
% , including number of qubits and qubit-layout \\
\hline
\end{tabular}
\caption{Benchmark-circuits for evaluating \projecttitle{}, adopted from the MQT Benchmark suite \cite{quetschlich2022mqt} and the Supermarq suite \cite{}. For each benchmark, we generate circuits wiht 4-100 qubits and respectively with $l$ layers or degree $d$.}
\label{tab:benchmarks} 
\end{table}

==> tables/interface.tex <==
\begin{table}[t]
\begin{tabular}{ |p{1.6cm}|p{6.2cm}| }
\hline
{\bf Function} & {\bf Description} \\
\hline
\textit{cut()} & Cuts a circuit into a virtual circuit with multiple fragments.  \\
% , including number of qubits and qubit-layout \\
\hline
\textit{vroute()} & Applies the virtual qubit-routing technique. \\
\hline
\textit{instantiate()} & Returns all the circuit-instantiations to run a virtual circuit \\
\hline
\textit{knit()} & Knits the results of the instantiations and returns the final result of the virtual circuit \\
\hline
\end{tabular}
\caption{The \projecttitle{} interface.}
\label{tab:interface} 
\end{table}


==> tables/metadata.tex <==
\begin{table}[t]
\begin{tabular}{ |p{1.9cm}|p{6cm}| }
\hline
{\bf Metadata} & {\bf Description} \\
\hline
\texttt{qpu} & Which QPU to run the qernel on \\
% , including number of qubits and qubit-layout \\
\hline
\texttt{shots} & Number of shots for sampling each qernel-instance \\
\hline
\texttt{init\_layout} & Mapping from logical to physical qubits on the \texttt{qpu} \\
\hline
\texttt{vgates} & How many virtual gates are allowed to be inserted \\
\hline
\end{tabular}
\caption{Metadata passed to a \texttt{run()} method of each \projecttitle{} layer.}
\label{tab:metadata} 
\end{table}


==> tables/params.tex <==
\begin{table}[t]
\begin{tabular}{ |p{1.9cm}|p{6cm}| }
\hline
{\bf Parameter} & {\bf Description} \\
\hline
\texttt{qpu\_infos} & Set of properties of the available QPUs \\
% , including number of qubits and qubit-layout \\
\hline
\texttt{overhead} & Maximum amount of virtual gates to use \\
\hline
\texttt{virt\_router} & Whether to use the virtual qubit-router until overhead limit is reached \\
\hline
\texttt{map\_strat} & Strategy to map fragments to QPUs \\
\hline
\end{tabular}
\caption{Parameters passed from the cut-decider to the virtual transpiler for creating a QPU-optimized virtual circuit.}
\label{tab:virt-trans-param} 
\end{table}

